Negative Data Augmentation

Data augmentation is often used to enlarge datasets with synthetic samples generated in accordance with the underlying data distribution. To enable a wider range of augmentations, we explore negative data augmentation strategies (NDA)that intentionally create out-of-distribution samples. We show that such negative out-of-distribution samples provide information on the support of the data distribution, and can be leveraged for generative modeling and representation learning. We introduce a new GAN training objective where we use NDA as an additional source of synthetic data for the discriminator. We prove that under suitable conditions, optimizing the resulting objective still recovers the true data distribution but can directly bias the generator towards avoiding samples that lack the desired structure. Empirically, models trained with our method achieve improved conditional/unconditional image generation along with improved anomaly detection capabilities. Further, we incorporate the same negative data augmentation strategy in a contrastive learning framework for self-supervised representation learning on images and videos, achieving improved performance on downstream image classification, object detection, and action recognition tasks. These results suggest that prior knowledge on what does not constitute valid data is an effective form of weak supervision across a range of unsupervised learning tasks.

==> abstract.tex <==
Self-supervised learning is an active research area for representation learning using unlabeled data. Most of the recent works focus on designing new loss functions or pretext tasks, paying little attention to the data transformations that build the foundation of learning representations. In this work, we propose a data transformation to induce learning of better deep models, without incorporating any auxiliary task or a new loss function. In our approach, we transform a natural image by degrading its spatial or structural consistency. These degraded examples are automatically created by dividing an image into a grid of patches and then randomly permuting them. 

We conduct experiments with such transformation in two scenarios, (a) we use such transformed real images as fake data for training BigGAN, and (b) we transform frames of a video to generate hard negative examples for self-supervised representation learning on videos using a CPC-inspired framework. Such fake data causes the discriminator of a GAN to learn the proper spatial structure of natural images, which in turn guides the generator to produce images with a more realistic structure. Similarly, introducing such hard-negatives for video representation learning causes the representations to encode spatial consistency as well. In spite of incurring no significant computation and being implemented in a few lines of code, our data transformation acheives state-of-the-art FID score for conditional/unconditional image generation and 
% improves strong baselines in GANs (conditional/unconditional) and
representation learning in videos. \ayush{This is a tentative abstract. I haven't included details about other transformations like stitching. Should we mention those as well here?}

==> background.tex <==
\section{Related Work}

\s{this section is not really useful. better to remove it and move the relevant snippets as intro in their respective sections}

\paragraph{Generative Adversarial Networks}. GANs have become one of the most important methods to learn generative models~\cite{goodfellow2014generative}. The idea behind GAN is the mini-max game. It uses a binary classifier, so-called the discriminator, to distinguish the data (real) versus generated (fake) samples. The generator of GAN is trained to confuse the discriminator to classify the generated samples as the real ones. By having the generator and discriminator competing with each other adversarially, they are able to improve themselves.  The end goal is to have the generator capture the data distribution. \s{move to nda gan} 

Let $G, D$ denote the generator and discriminator of the GAN. Further let $p_d, p_g$ denote the real data and generated distribution respectively. Then the GAN objective is defined as the following - 
\begin{equation}
    \min\, \max_{G,D} \E_{x \sim p_d}\left[\log(D(x))\right] + \E_{x \sim p_g}\left[\log(1 - D(x))\right]
    \label{eq:GAN}
\end{equation}
% $$min\, max_{G,D} E_{x \sim p_d}\left[log(D(x))\right] + E_{x \sim p_g}\left[log(1 - D(x))\right]$$


\paragraph{Self-supervised learning from images} A variety of pretext tasks have been proposed to learn representations from unlabelled images. Some tasks leverage the spatial context in images~\cite{doersch2015unsupervised} to train CNNs. Others create pseudo classification labels by artificial rotations~\cite{gidaris2018unsupervised}, or clustering features~\cite{caron2018deep}. Other tasks include colorization~\cite{zhang2016colorful}, predicting features~\cite{oord2018representation}, inpainting~\cite{pathak2016context} and solving jigsaw puzzles~\cite{noroozi2016unsupervised}. 

\paragraph{Self-supervised learning from videos}
Modern cameras capture videos with large frame rates. This makes the annotation of such videos even more time-consuming and costly than annotating a single image. For this reason, unsupervised learning for computer vision tasks in videos have been studied extensively recently~\cite{ahsan2019video,wang2018video,han2019video,kim2019self}. Some of the tasks that use the space dimension of the image have been extended to the space-time dimensions of videos by crafting equivalent tasks. Similar to image recognition, using spatial displacement of image patches have been used for puzzle solving as a pretext task in videos. Other tasks include predicting geometric transformations~\cite{jing2018self}, making use of temporal dimension of videos to learn representations by predicting shuffled frames!\cite{misra2016shuffle}, arrow of time~\cite{wei2018learning}, etc.


% Unlike solving jigsaw puzzle in a pretext task in both videos and images, we propose the use of jigsaw images as a negative data augmentation method.

\paragraph{Data Augmentation} 
Data Augmentation has become a prominent and indispensable technique in deep learning to overcome the paucity of training dataset by producing more labeled samples cheaply, allowing the model generalize to unseen datapoints. A common technique employed is to ensure that the output of the model remains invariant to such data augmentation techniques. Semantic preserving transformations such as Random Crop, Image mirroring~\cite{krizhevsky2012imagenet,he2016deep} and color whitening are commonly used. Mathematically speaking, such semantic preserving stochastic transformations take $(x, y)$ from the joint data distribution $p(x, y)$ and produce a new point in the support of $p(x, y)$. Semantic distorting augmentations such as Mixup~\cite{zhang2017mixup}, Cutout~\cite{devries2017improved}, CutMix~\cite{yun2019cutmix} have been shown to achieve even better results for the image classification task. However, using such semantic distorting augmentations to ensure transformational invariance can bias the generator to generate such out of distribution images too. In this work, we show a clear framework to leverage such spatially corrupting augmentations to improve the performance of GANs by pitting them as fake data. \s{move some of this to nda section 3}

% \paragraph{Learning Representations on Images} Recently, unsupervised learning has been a very active area of research as annotating large amount of images with human labels is time-consuming and costly~\cite{kolesnikov2019revisiting,mahajan2018exploring,le2013building}. One major area within unsupervised learning focuses on designing pretext tasks such as colorization~\cite{zhang2016colorful}, jigsaw puzzle solving~\cite{noroozi2016unsupervised}, and rotation angle prediction~\cite{gidaris2018unsupervised}. The jigsaw puzzle, our focus in this study, relies on spatial displacement of image patches. In particular, all the jigsaw puzzle related studies model input by random spatial displacement of image patches and formulate the task of predicting displacement order as a pretext task ~\cite{noroozi2016unsupervised,kim2018learning,carlucci2019domain}.~\cite{noroozi2016unsupervised} is the first study proposing the idea of using jigsaw puzzles as a pretext task. They divide the images into 3x3 disjoint patches, shuffle and passes 
% them through the CNN with shared weights to get patch representations. The representations across the patches are then concatenated to use as input to an MLP model predicting the order of the patches.~\cite{carlucci2019domain}, on the other hand, utilizes jigsaw puzzle solving as an auxiliary task to more strictly regularize CNNs for better domain generalization. Unlike~\cite{noroozi2016unsupervised}, they use no gap in between the neighboring patches and a smaller permutation space. They formulate the auxiliary task as a classification task where the CNN classifies spatially corrupted input image into one of the permutation indices.



==> nda.tex <==
\section{Negative Data Augmentation}
\subsection{Negative Sampling}
% Let $p_{real}$ denote the real data distribution and $x \sim p_{real}$ denote a sample from it. Let $T(x)$ be a stochastic negative data augmentation that produces a new point outside of the support of $p_{real}$. Let $\overline{p}$ be the distribution induced by applying the stochastic transformation $T$ over the samples $x$ in $p_{real}$. $p_{real}$ and $\overline{p}$ satisfy the following relation: $supp(P) \cap supp(\overline{P}) = \emptyset$.
% Intuitively, we also want the support of $\overline{p}$ to be close to the support of $p_{real}$ in order for the transformed samples to be useful.
Let $p$ denote the data distribution of interest and $x \sim p$ denote a sample from it. Let $x'$ be a new point sampled from $\overline{p}$ lying outside of the support of $p$. Under these conditions $p$ and $\overline{p}$ satisfy the following relation: $supp(P) \cap supp(\overline{P}) = \emptyset$. To be able to learn more useful information, we also want the support of $\overline{p}$ to be close to the support of $p$. In this concept, any point sampled from $p$ and $\overline{p}$ can be used in a variety of range tasks utilizing contrastive loss function and GANs.

\begin{figure*}[!h]
\centering
    \includegraphics[width=5cm]{example-image-a}
    \caption{Overview Diagram}
    \label{fig:overview}
\end{figure*}

\subsection{Negative Sampling using Data Augmentation}
Data transformations, $\phi$, is generally used to collect a positive pair $x^'$ of an image $x$ sampled from $p$~\cite{he2019momentum}. This concept has been used to perform data augmentation to avoid overfitting in supervised learning, regularize GANs and unsupervised representation learning with contrastive loss functions. On the other hand, it has not been utilized to generate a negative image $x^'$ using its own image $x$ sampled from $p$. As mentioned previously, we want the distribution $\overline{p}$ with a close support to $p$ while meeting the following relation: $supp(P) \cap supp(\overline{P}) = \emptyset$ to to learn more useful representations. In this study, we utilize some of the data augmentations to generate samples $x'=\phi(x)$ with the goal of using them as negative samples. However, we want to highlight not all the data transformations can be applied to create negative samples as they might induce $\overline{p}$ overlapping with with the support of $p$. For this reason, in particular we investigate the transformations that corrupts the original images spatially to meet our two conditions: (1) $supp(P) \cap supp(\overline{P}) = \emptyset$ and (2) close support between $p$ and $\overline{p}$. Additionally, by contrasting representations learned from spatially corrupted images, $x^{'}=\phi(x)$, and original images $x$, we can learn semantically consistent representations. In the next section, we detail our transformations used to generate negative samples.


% \subsection{Why NDA?}
% \ayush{Not sure where to put this section. Putting it here for time being. Will also trim it a bit.}
% It is easier for GANs to learn to generate texture elements and small scale local features than to generate objects with a realistic structure. \cite{liu2018intriguing} showed that a CNN does not perform well in tasks related to spatial reasoning by default. Traditional convolutional GANs generate high-resolution details as a function of only spatially local points in lower-resolution feature maps. Therefore, we posit that a CNN is not readily amenable to learning feature representations that capture global structural details in images. 

% We believe our proposed data transformation encourages a CNN-based discriminator to learn global structural consistency more directly. Given that the key learning signal for training the generator comes from the discriminator, the losses against which the discriminator is trained implicitly guide the effective training of the generator. Thus, training the discriminator to learn useful global spatial consistencies may produce better generators. Using only a single signal (real/fake) to guide the generator to learn the high-dimensional, complex data distribution and at the same time encode global image information is very challenging. We propose to generate fake images by transforming real images. We divide a real image into a $K \times K$ grid and permute the patches to generate a structurally corrupted (fake) image. Our intuition is that posing such structurally corrupted real images as fake data will help the discriminator to be better at capturing global consistency. This improved discriminator can indirectly signal the generator to produce more structurally coherent images. Our proposed transformation to create fake data thus provides a stronger signal on several datasets and we achieve improved image generation results, using Frechet inception distance (FID), against strong baselines. Not only does our approach improve generation performance in the unconditional GAN setting, but it also improves performance in class conditional GANs.  

\subsection{Types of Negative Data Augmentation for Images}

\begin{figure*}[!h]
\centering
    \includegraphics[width=3cm]{example-image-a}
    \caption{Types of Augmentation}
    \label{fig:types}
\end{figure*}

In the following, we describe several types of negative data augmentation over images of size $H \times W$.

\begin{description}
    \item[Jigsaw-$K$] \cite{noroozi2016unsupervised} We partition the image into $K \times K$ patches of size $(H/K) \times (W/K)$ (where $K$ is divisible by $H$ and $W$), indexed by $[1, \ldots, K\times K]$; then we shuffle the image patches according to random permutations (different from the original order) to produce NDA images.
    \item[Stitching] We stitch the NDA image from two equal-sized patches of two images, either horizontally ($H/2 \times W$) or vertically ($H \times W/2$), chosen uniformly at random.
    \item[Cutout / Cutmix] We select a random patch in the image where we randomly select height, width and location from \js{height, width, location distributions} respectively. To construct NDA images, this patch is replaced with zero values~\cite{devries2017improved} (cutout), or the pixel values of another image at the same location~\cite{yun2019cutmix} (cutmix). 
    \item[Mixup-$\alpha$] NDA images are constructed from linear interpolation between two images $\vx$ and $\vy$~\cite{zhang2017mixup}: $\lambda \vx + (1 - \lambda) \vy$, where $\lambda$ is selected from $\mathrm{Beta}(\alpha, \alpha)$. $\alpha$ is chosen to be large so that the distribution has high density at 0.5.
    
    %\js{which distribution? this matters because if $\lambda$ is close to 1 then we don't have negative sample}\ayush{we are sampling from beta distribution.}\js{which parameters for beta? using 1, 1, is very different from using 4, 4}\ayush{currently using 1,1. What would you suggest? We can rerun the experiment.}\js{I would suggest larger hyperparameters, since it leads to samples more centered on the mean. wikipedia has some nice visualizations, i feel like 1, 1, is not going to cut it because it is uniform}
    \item[Other datasets] NDA images are sampled from other datasets, or other classes in the same dataset.
\end{description}

% \paragraph{Jigsaw} - We divide the image into a $K \times K$ grid, and then randomly permute the grid patches. For videos we apply the same permutation to all frames in a video.

% \paragraph{Stitching} - For each image $x$ in a batch, we select another image $y \neq x$, and then stitch the two images. For stitching we either merge the top half of x with bottom half of y, or merge the left half of x with right half of y.

% \paragraph{Cutout} - Similar to ~\cite{devries2017improved}, we mask out a random patch in an image. The patch size is randomized during training.

% \paragraph{Cutmix} - As in ~\cite{yun2019cutmix}, we randomly paste the patch of an image $y$ onto an image $x$. Again, the patch size is randomized.

% \paragraph{Mixup} As proposed in ~\cite{zhang2017mixup}, we do linear interpolations between two images, and use the interpolated image as a negative data.

%define negative data augmentation. transformation that maps data to something out of support. intuitively, shouldn't be too not too far away from the support to be useful.

% introduce various forms of negative data augmentation (for images). jigsaw, noise, other dataset. 


==> related_work.tex <==
\section{Related Work}
\subsection{Spatial structure of images for learning}

\subsection{Data Augmentation for GANs}

\subsection{Jigsaw for Unsupervised Learning}


==> sections/1_introduction.tex <==
\section{Introduction}
Data transformations have been critical in supervised learning~\cite{chen2020simple,he2019momentum,oord2018representation} to enlarge datasets (data augmentation) by applying transformations such as rotation, blurring, cropping etc. to the already annotated images. Transformations employed for data augmentation have also played a key role to the success of recent representation learning methods in unsupervised learning with contrastive loss functions~\cite{chen2020simple,he2019momentum} and pre-text tasks~\cite{gidaris2018unsupervised,zhang2016colorful,noroozi2016unsupervised,kim2018learning,wei2019iterative,ahsan2019video}. Finally, data transformations have been used to more strictly regularize GANs by ensuring that the classifier output remains unaffected for an image under transformations~\cite{zhang2019consistency,zhao2020improved,antoniou2017data}. 
%All these methods provide an inductive bias to the model, which encourages invariances across the transformations~\cite{jaiswal2018unsupervised,antoniou2017data}.
% Semantically inconsistent image transformations, on the other hand, mostly have been utilized in pre-text tasks for unsupervised representation learning. A widely used transformation, called \emph{jigsaw} that spatially dislocates the image patches, has been used to design puzzle solving pre-text tasks ~\cite{noroozi2016unsupervised,kim2018learning,wei2019iterative,ahsan2019video} and auxiliary tasks for improving domain adaptation~\cite{carlucci2019domain}.

% \ayush{First line of this para is same as last line of prev. para?} 
Data augmentation enforces invariances and other inductive biases by creating more in-distribution samples from in-distribution data through data transformations~\cite{jaiswal2018unsupervised,antoniou2017data}. Under such transformations, existing augmentation techniques encourage capturing relevant representations in both supervised and unsupervised learning setup. In this study, on the other hand, we propose to inject different inductive biases by creating out-of-distribution samples from in-distribution through task specific transformations.
%\ayush{We propose to inject different inductive biases by creating out-of-distribution (OOD) samples from in-distribution through task specific transformations?}. 
In other words, we utilize the representations from out-of-distribution (OOD) data to better guide the representations on the original data. In particular, contrary to existing data augmentation techniques, we encourage the disparity between the representations from the original and transformed input. Although, we finally care about the performance over in-distribution samples, using OOD samples helps a model to better chart out the data-distribution boundary. Under this hypothesis, we then name such augmentation strategy \emph{Negative Data Augmentation} (NDA) and utilize them in generative modeling and unsupervised learning with contrastive loss functions~\cite{chen2020simple,he2019momentum,oord2018representation}.

% Existing augmentation techniques argue that good representations should capture the relevant information under semantic preserving transformations. Some of these semantic preserving transformations include Gaussian noise addition, rotation, and flipping have been widely used in regularizing generative modeling, unsupervised representation learning and augmenting small-size datasets in supervised learning~\cite{chen2020simple,he2019momentum,oord2018representation}. Contrary to such semantic preserving (\emph{positive}) transformations we explore semantic non-preserving (\emph{negative}) transformations, that intentionally destroy the semantics of input to inject a different inductive bias to the model. 

The negative data augmentation is critical in practice as existing approaches in generative modeling and unsupervised representation learning are typically oblivious of the model behavior under out-of-support data. For example, a generative adversarial network (GAN) trained on images with 2 objects may \emph{over-generalize} and generate images with 1 or 3 objects~\cite{zhao2018bias}, and there is no explicit way of preventing such issues with the existing augmentation paradigm; if we provide \textit{negative} samples with 1 or 3 objects, we may bias the behavior of the model to a more desirable outcome.
In general, such artificially created out-of-distribution samples can then be applied as \textit{negatively augmented data} to generative modeling, and unsupervised representation learning as they can characterize the data distribution in a way that we can avoid undesirable behaviour over such OOD samples.

% \js{so maybe we can modifyragraph 2 and 3 to be like this: image transformationpa  and relevant pre-text tasks has seen wide use in generating semantic preserving samples for GANs and representation learning, but we are interested in the model behavior on out-of-distribution samples (which data augmentation does not address, i think this issue is quite important), so we generate non semantic preserving samples, negative data-augmentation, to address these issues}
% \s{expand this paragraph, use logic from section 3 and abstract}

In this study, we develop a clear framework for introducing such negative data augmentations and show its effectiveness for two classes of task: (a) image generation using generative adversarial networks, and (b) representation learning for images and videos via contrastive learning. For GANs, under suitable conditions, we theoretically show that with our proposed approach, the optimal solution for the generator of a GAN~\cite{goodfellow2014generative} still recovers the underlying true distribution. NDA biases the learning process of the GAN by directly providing supervision on what should not be generated by explicitly specifying such samples as OOD data. 
% Without NDA, the generator may ``over-generalize'' beyond the empirical distribution to include undesired samples.
\se{explain in words: provide supervision in terms of what samples not to generate (what we know is ood)}\ayush{Added}
Our technique is simple to use and quite effective and we show that that applying this technique on top of existing GAN models (conditional/unconditional) leads to new state-of-the-art results as measured by Frechet Inception Distance. We further show that training a GAN with NDA modifies the behaviour of the discriminator over OOD data, thereby resulting in an improved performance over  (a) anomaly detection, and (b) representation learning.
On the other hand, for representation learning, we also show that under suitable assumptions, our approach encourages the representations of in-support data to become disjoint from the representations of OOD data. Empirically, we show that applying NDA over existing contrastive learning based approaches for images and videos improves performance over downstream tasks such as image-classification and action-recognition.

%\s{discuss in words the representation learning stuff}\abhishek{Done}

In summary, our contributions are summarized as follows: 

\begin{itemize}
    \item We propose \textit{Negative Data Augmentation} strategy for GANs and Contrastive Representation Learning by explicitly providing inductive bias over OOD data thus regularizing behaviour over in-support data.
    
    \item We investigate the desired effects of NDA over two toy tasks (using CLEVR and Dots datasets) where we empirically show that NDA biases the generator of a GAN to avoid \emph{over-generalization} to undesired samples.
    % additional bias to the generator. This prevents the generator from generating out-of-distribution samples that a normal GAN usually learns to generate.
    
    \item We conduct extensive experiments with BigGAN to demonstrate that our technique leads to new state-of-the-art results for unconditional/conditional image generation as measured by Frechet Inception Distance. We also show improvements in the Discriminator for (a) anomaly detection, and (b) representation learning.
    
    \item We show that simply applying the proposed technique to Contrastive Learning methods for images and videos can further boost the boost the performance on downstream tasks like image classification and action recognition.
\end{itemize}

%\ayush{General intro about importance of global information}
%Visual information in the world comes with local and global spatial/structural consistencies and learning a good representation from them is important both for human perception and machine learning systems. To learn a good representation from visual information, we argue that, it is essential to encode global structural consistency as well apart from local consistencies. \burak{this does not align with abstract. In the abstract, we do not suggest that we are learning global representations. I think we can start with --> the performance of convolutional neural networks (CNNs) depend on the quality and amount of labeled images. In many areas within computer vision, it is time-consuming and financially costly to collect labels and images to build a large scale dataset [cite]. For this reason, image transformations such as rotation, blurring, blocking, jigsaw etc. has been critical in the fields of data augmentation and unsupervised learning [cite]. In this study, we investigate the effect of transformations that spatially corrupts the images in training the generative models, and learning representations without supervision for image and video understanding.} 



% Let us denote the data distribution by $p_d$ and the generated distribution by $p_g$. 
% For a given real image $x_r \sim p_d$, we create a permuted version of it, by dividing the image in a k*k patch and then permuting the patches. Let us denote the permuted image by $x_p$. We have $x_p = T(x_r), x_r \sim p_d$, where $T$ is the jigsaw transformation function.\\
% Further, let $x_n \sim N(0,1)$ be the samples from the gaussian distribution. For an optimal discrimnator $D^{*}$, the output of discriminator is given as $D^*(x) = \frac{p_d(x)}{p_d(x) + p_g(x)}$ (\textbf{Whats the optimal discriminator for a GAN trained with Hinge loss ?}). We want to explore the behaviour of the discriminator over samples that are outside the support of the discriminator. Specifically, we explore For a BigGAN model trained over CIFAR-10, we find its behaviour over such out-of-support samples to be pretty aberrant.

% \begin{figure}[h]
% \centering
% \includegraphics[width=2.5in,height=2.0in]{sections/images/jigsaw_2disc_diff.png}
% \caption{Histogram of D($x_r$) - D($x_p$)}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=2.5in,height=2.0in]{sections/images/noisedisc.png}
% \caption{Histogram of D($x_n$)}
% \end{figure}

% \textbf{Our aim is to increase the support of the discriminator, to samples outside the generated and real distribution, in a way that it makes it easier for the generator to model the true distribution.}

% Original GAN objective - 
% $$min\, max_{G,D} E_{x \sim p_d}\left[log(D(x))\right] + E_{x \sim p_g}\left[log(1 - D(x))\right]$$

% New GAN objective - 
% $$min\, max_{G,D} E_{x \sim p_d}\left[log(D(x))\right] + E_{x \sim p_g}\left[log(1 - D(x))\right] + E_{x \sim p_d}\left[log(1 - D(T(x)))\right]$$

%     \begin{itemize}
%     \item augmentation with ``fake'' data constructed from self-supervision
%     \item why does this work? changes the objective and the corresponding equilibrium solution
%     \item what type of augmentation have we considered> Jigsaw, stitching, jigsaw shift (curriculum learning)
%     \item experiments: GAN generation, DPC, use discriminator for outlier detection
% \end{itemize}




==> sections/5_experiments.tex <==
%\section{Experiments}



==> sections/intro_old.tex <==
\section{Introduction}
Data augmentation strategies for  synthesizing new datapoints in a way that is consistent with an underlying task are extremely effective in both supervised and unsupervised learning~\cite{chen2020simple,he2019momentum,oord2018representation,zhang2016colorful,noroozi2016unsupervised,asano2019critical}. Because they operate at the level of samples, they can be combined with most learning algorithms.
They allow for the incorporation of prior knowledge (inductive bias) about properties of typical samples from the underlying data distribution % (in-distribution)
~\cite{jaiswal2018unsupervised,antoniou2017data}, 
e.g., by leveraging invariances to produce additional "positive" examples of how a task should be solved.
%e.g., that an image's label should be invariant to small color changes or shifts. 
%Because they operate at the level of samples, they are easy to incorporate in most learning algorithms.
%However, coming up with effective data augmentation strategies is task-dependent and generally non-trivial \kristy{cite} \burak{I think this statement gives the impression that we are proposing a solution to make them task-agnostic. We might better finish with inductive bias and carry on with introducing wider range of bias,}. 
%Methods for automatically discovering them are an active area of research~\cite{cubuk2019autoaugment}.

To enable users to specify an even wider range of inductive biases,  
%\kristy{there is a disconnect with the proposed problem above (coming up with data augmentation strategies is task-dependent/hard) and the solution (specifying a wider range of biases to choose from). should make this clear}, 
we propose to leverage an alternative
and complementary 
%\sj{unclear it's alternative and complementary to what?} 
source of prior knowledge  
%about the underlying distribution
intuitively corresponding to ways in which a task should \emph{not} be solved. 
%
%that is complementary to existing approaches. \kristy{what are these existing approaches and why was it necessary to look at complementary approaches? answering this Q will also clear up the above point as well as the problem statement in the abstract} 
We formalize this intuition by assuming access to a way of generating samples that are guaranteed to be out-of-support for the data distribution (out-of-distribution samples), which we call a  \emph{Negative Data Augmentation} (NDA). 
\begin{comment}
While task-specific, we argue that NDA samples exist and are easy to define for common data modalities such as natural images, which are 
%believed to be 
supported on low-dimensional manifolds \cite{fefferman2016testing}.
%, where it is sufficient to create NDA samples by destroying spatial/structural coherence. 
Focusing on natural images and videos, we provide generic NDA strategies building on known transformations from the literature that intentionally destroy the spatial coherence of an image~\cite{noroozi2016unsupervised,devries2017improved,yun2019cutmix}, such as the Jigsaw puzzle transformation.
\end{comment}
We then propose new methods to use NDA samples for training generative adversarial networks (GANs) and representation learning. 
%\kristy{up to this sentence, the flow of this paragraph is weak. it should be more like: (to address challenge X, we propose NDA as an alternative data augmentation strategy) -> (NDA consists of leveraging an alternative source of prior knowledge...) -> (to do so, we assume access to...). basically, the statement of what you're doing should come first, then followed by details. right now it's more like details first then what you are doing, which can be confusing for the reader to follow}
%Although in most cases we only care about performance for in-distribution samples,
Intuitively, negative out-of-distribution (OOD) samples can 
%still 
be leveraged as a useful inductive bias because they provide information about the support of the data distribution to be learned by the model. For example, in a density estimation problem we can bias the model to avoid putting any probability mass in regions which we know a-priori should have zero probability. This can be an effective prior if the negative samples cover a sufficiently large area. 
%\kristy{this intuition was helpful} 
%\sj{This argument didn't feel convincing because negative samples only cover a extremely small region outside of support. I think it's hard to believe that the performance improvement comes from additional information about the support. e.g. if you just use Gaussian noise as the negative sample it wouldn't work no?} 
 %\abhishek{we have addressed this point in section 2.1, I don't think we need to explain it here}
%Under this hypothesis, we then name such augmentation strategy \emph{Negative Data Augmentation} (NDA) and utilize them in generative modeling and unsupervised learning with contrastive loss functions~\cite{chen2020simple,he2019momentum,oord2018representation}.

%\sj{The structure is not super clear here. I'm assuming you want to say: we discuss the general technique of negative samples, then apply it to applications: GAN, anomaly detection and representation learning. Some transitional statements can help.} 
Building on this intuition, we introduce a new GAN training objective where we use 
%out-of-distribution data obtained via
NDA as an additional source of fake data for the discriminator. 
Theoretically, we can show that if the NDA assumption  
%\kristy{if the procedure is valid? or the assumption?} 
is valid, 
%(i.e., the NDA and data supports are truly disjoint), 
optimizing this objective will still recover the data distribution in the limit of infinite data. 
However, in the finite data regime, there is a need to generalize beyond the empirical distribution~\cite{zhao2018bias}. By explicitly providing the discriminator with samples we want to avoid, we are able to bias the generator towards avoiding undesirable samples thus improving generation quality. 
%generalization of the dataset %\kristy{(confusing)}
%put probability mass where it shouldn't. 
%\sj{This seems strange, since the discriminator is trained on the generated fake samples. So any fake sample should theoretically be detected by the discriminator, and thus avoided. I think you might have intended to argue about the empirical weakness observed in our neurips paper, but I don't that flavor came out from the text. }
%
%This idea can be applied to any existing GAN.
In practice, we propose to interpret known transformations from the literature that intentionally destroy the spatial coherence of an image~\cite{noroozi2016unsupervised,devries2017improved,yun2019cutmix}, such as the Jigsaw puzzle transformation, as NDAs. 
%and using the generic augmentations described above
Combined with existing GANs, 
we achieve new state of the art FID \cite{heusel2017gans} scores for conditional/unconditional image generation on CIFAR-10/100. 
We further show that training a GAN with NDA modifies the behavior of the discriminator over OOD data, and yields improved performance in anomaly detection. 
%\sj{This point seems sketchy. The statement seems to imply that modified behavior *causally* improves anomaly detection performance. Maybe if there is no good justification this statement should be downplayed to avoid skepticism.}
% For GANs, under suitable conditions, we theoretically show that with our proposed approach, the optimal solution for the generator of a GAN~\cite{goodfellow2014generative} still recovers the underlying true distribution. NDA biases the learning process of the GAN by directly providing supervision on what should not be generated by explicitly specifying such samples as OOD data. 

% Our technique is simple to use and quite effective and we show that that applying this technique on top of existing GAN models (conditional/unconditional) leads to new state-of-the-art results as measured by Frechet Inception Distance. We further show that training a GAN with NDA modifies the behaviour of the discriminator over OOD data, thereby resulting in an improved performance over  (a) anomaly detection, and (b) representation learning.


% Without NDA, the generator may ``over-generalize'' beyond the empirical distribution to include undesired samples.

% \js{so maybe we can modifyragraph 2 and 3 to be like this: image transformationpa  and relevant pre-text tasks has seen wide use in generating semantic preserving samples for GANs and representation learning, but we are interested in the model behavior on out-of-distribution samples (which data augmentation does not address, i think this issue is quite important), so we generate non semantic preserving samples, negative data-augmentation, to address these issues}
% \s{expand this paragraph, use logic from section 3 and abstract}


Furthermore, we propose a way of leveraging NDA for unsupervised representation learning. We propose a new contrastive predictive coding~\cite{he2019momentum,han2019video} (CPC) objective that encourages the distribution of representations corresponding to in-support data to become disjoint from that of NDA data.  
%\kristy{what does it mean for representations to become disjoint? e.g. if i have real-valued vectors},
As in the previous GAN example, enforcing  disjointedness will bias the learned representation in a certain way, potentially improving performance. 
%by preventing solutions with overlap we hope to 
%which is important in safety-critical applications such as anomaly detection. 
%\sj{Why is this beneficial?} 
Empirically, we show that applying NDA with our proposed transformations (e.g., forcing the representation of normal and jigsaw images to be disjoint)
%over existing contrastive learning approaches for images and videos 
improves performance in downstream tasks such as image-classification, action-recognition, and anomaly detection. These results suggest that NDA has much potential to improve a variety of unsupervised learning techniques. 
%\kristy{a lot of strong empirical results! wow}
%for generative models and representation learning.
% These results suggest that prior knowledge on what does not constitute valid data is an effective form of weak supervision across a range of unsupervised learning tasks. \abhishek{Abstract also contains the same line, need to modify this}

%\s{discuss in words the representation learning stuff}\abhishek{Done}


%\ayush{General intro about importance of global information}
%Visual information in the world comes with local and global spatial/structural consistencies and learning a good representation from them is important both for human perception and machine learning systems. To learn a good representation from visual information, we argue that, it is essential to encode global structural consistency as well apart from local consistencies. \burak{this does not align with abstract. In the abstract, we do not suggest that we are learning global representations. I think we can start with --> the performance of convolutional neural networks (CNNs) depend on the quality and amount of labeled images. In many areas within computer vision, it is time-consuming and financially costly to collect labels and images to build a large scale dataset [cite]. For this reason, image transformations such as rotation, blurring, blocking, jigsaw etc. has been critical in the fields of data augmentation and unsupervised learning [cite]. In this study, we investigate the effect of transformations that spatially corrupts the images in training the generative models, and learning representations without supervision for image and video understanding.} 



% Let us denote the data distribution by $p_d$ and the generated distribution by $p_g$. 
% For a given real image $x_r \sim p_d$, we create a permuted version of it, by dividing the image in a k*k patch and then permuting the patches. Let us denote the permuted image by $x_p$. We have $x_p = T(x_r), x_r \sim p_d$, where $T$ is the jigsaw transformation function.\\
% Further, let $x_n \sim N(0,1)$ be the samples from the gaussian distribution. For an optimal discrimnator $D^{*}$, the output of discriminator is given as $D^*(x) = \frac{p_d(x)}{p_d(x) + p_g(x)}$ (\textbf{Whats the optimal discriminator for a GAN trained with Hinge loss ?}). We want to explore the behaviour of the discriminator over samples that are outside the support of the discriminator. Specifically, we explore For a BigGAN model trained over CIFAR-10, we find its behaviour over such out-of-support samples to be pretty aberrant.

% \begin{figure}[h]
% \centering
% \includegraphics[width=2.5in,height=2.0in]{sections/images/jigsaw_2disc_diff.png}
% \caption{Histogram of D($x_r$) - D($x_p$)}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=2.5in,height=2.0in]{sections/images/noisedisc.png}
% \caption{Histogram of D($x_n$)}
% \end{figure}

% \textbf{Our aim is to increase the support of the discriminator, to samples outside the generated and real distribution, in a way that it makes it easier for the generator to model the true distribution.}

% Original GAN objective - 
% $$min\, max_{G,D} E_{x \sim p_d}\left[log(D(x))\right] + E_{x \sim p_g}\left[log(1 - D(x))\right]$$

% New GAN objective - 
% $$min\, max_{G,D} E_{x \sim p_d}\left[log(D(x))\right] + E_{x \sim p_g}\left[log(1 - D(x))\right] + E_{x \sim p_d}\left[log(1 - D(T(x)))\right]$$

%     \begin{itemize}
%     \item augmentation with ``fake'' data constructed from self-supervision
%     \item why does this work? changes the objective and the corresponding equilibrium solution
%     \item what type of augmentation have we considered> Jigsaw, stitching, jigsaw shift (curriculum learning)
%     \item experiments: GAN generation, DPC, use discriminator for outlier detection
% \end{itemize}




==> sections/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

